Automatic Correction of Human Translations

We introduce translation error correction (TEC), the task of automatically correcting human-generated translations. Imperfections in machine translations (MT) have long motivated systems for improving translations post-hoc with automatic post-editing. In contrast, little attention has been devoted to the problem of automatically correcting human translations, despite the intuition that humans make distinct errors that machines would be well-suited to assist with, from typos to inconsistencies in translation conventions. To investigate this, we build and release the Aced corpus with three TEC datasets. We show that human errors in TEC exhibit a more diverse range of errors and far fewer translation fluency errors than the MT errors in automatic post-editing datasets, suggesting the need for dedicated TEC models that are specialized to correct human errors. We show that pre-training instead on synthetic errors based on human errors improves TEC F-score by as much as 5.1 points. We conducted a human-in-the-loop user study with nine professional translation editors and found that the assistance of our TEC system led them to produce significantly higher quality revised translations.

==> sections/22-error-and-edit.tex <==
\begin{table*}
\begin{subtable}[t]{.51\textwidth}
\centering
\small
\begin{tabular}[t]{lccc|c}\toprule
& \asics{} & \emerson{} & \digitalocean{} & APE \\
\midrule
Monolingual: technical & 12 & 16 & 22 & 16 \\
Monolingual: grammar  & 41 & \phantom{0}4 & \phantom{0}2 & \phantom{0}6 \\
Monolingual: fluency  & 23 & \phantom{0}0 & 20 & 74 \\
Bilingual             & 22 & 70 & 32 & \phantom{0}5 \\
Preferential          & \phantom{0}8 & 24 & 40 & \phantom{0}6 \\
\bottomrule
\end{tabular}
\caption{Percentages of erroneous sentences that contain at least one error of each type for \asics{}, \emerson{}, \digitalocean{}, and the dev set of the WMT 2021 APE shared task. As a task, APE exhibits many more fluency errors than TEC.}
\label{tab:error-breakdown}
\end{subtable}%
\hfill%
\begin{subtable}[t]{.48\textwidth}
\centering
\flushright
\small
\begin{tabular}[t]{llccc}\toprule
 & & \asics{} & \emerson{} & \digitalocean{} \\
\midrule
\multirow{2}{*}{Train} & Total Edits & 606 & 1436 & 1212 \\
                        & Unique Edits & 418 & \phantom{0}486 & \phantom{0}940 \\
\midrule
\multirow{2}{*}{Dev}  & Total Edits & 246 & \phantom{0}381 & 1004\\
                    & \% in train & \phantom{0}14 & \phantom{0}\phantom{0}63 & \phantom{00}21 \\
\midrule
\multirow{2}{*}{Test}  & Total Edits & 287 & \phantom{0}364 & \phantom{0}766 \\
                    & \% in train & \phantom{0}23 & \phantom{00}60 & \phantom{00}21 \\
\bottomrule
\end{tabular}
\caption{Edit and edit overlap statistics for each \datasetname{} dataset: total number of edits, unique edits in each train split, and percentage of total edits in each dev and test split that appear in the train split.}
\label{tab:edit-overlap}
\end{subtable}%

\end{table*}
